Hierarchical Fault-Tolerant Coverage Control for an Autonomous Aerial Agent

Fault-tolerant coverage control involves determining a trajectory that enables an autonomous agent to cover specific points of interest, even in the presence of actuation and/or sensing faults. In this work, the agent encounters control inputs that are erroneous; specifically, its nominal controls inputs are perturbed by stochastic disturbances, potentially disrupting its intended operation. Existing techniques have focused on deterministically bounded disturbances or relied on the assumption of Gaussian disturbances, whereas non-Gaussian disturbances have been primarily been tackled via scenario-based stochastic control methods. However, the assumption of Gaussian disturbances is generally limited to linear systems, and scenario-based methods can become computationally prohibitive. To address these limitations, we propose a hierarchical coverage controller that integrates mixed-trigonometric-polynomial moment propagation to propagate non-Gaussian disturbances through the agent's nonlinear dynamics. Specifically, the first stage generates an ideal reference plan by optimising the agent's mobility and camera control inputs. The second-stage fault-tolerant controller then aims to follow this reference plan, even in the presence of erroneous control inputs caused by non-Gaussian disturbances. This is achieved by imposing a set of deterministic constraints on the moments of the system's uncertain states.

==> approach.tex <==
\section{Robust Hierarchical Coverage Control} \label{sec:approach}
In this section, we show how we have addressed the challenges discussed in Sec. \ref{sec:problem} by designing a robust hierarchical coverage controller. In the first stage (i.e., Sec. \ref{ssec:stage1}), the problem in \eqref{eq:P1} is reformulated as a disturbance-free rolling horizon model predictive control problem (MPC), generating finite-length look-ahead coverage plans. This controller jointly optimizes the agent's mobility and camera control inputs via mixed integer quadratic programming, producing a reference coverage plan for the second-stage controller to track. In the second stage (i.e., Sec. \ref{ssec:stage2}), a robust controller is developed, employing exact uncertainty propagation techniques to propagate the disturbance through the agent's dynamics. This allows for the computation of constraints on the moments of the agent's uncertain states, ensuring coverage at specified probability levels.


\subsection{Stage-1: Coverage Reference Plan} \label{ssec:stage1}
The first-stage controller, as formulated in \eqref{eq:P2}, is designed as a rolling horizon MPC. In this setup, the agent computes finite-length look-ahead coverage trajectories $\boldsymbol{x}^1_{t+\tau+1|t}$ for $\tau \in \{0,..,T^1-1\}$. Here, the notation $x_{\tau|t}$ represents the predicted state of the agent at future time-step $\tau \geq t$, as calculated at the current time-step $t$. This coverage planning process is executed iteratively across multiple time-steps $t$, where the first set of predicted control inputs $\boldsymbol{u}^1_{t|t} \in \mathcal{U}^1$ in the sequence is executed at the subsequent time-step. Following this, the agent transitions to its new state, and the optimization cycle described above is repeated for the next time-step, now over a shifted planning horizon of $T^1$ time-steps.


\begin{algorithm}[h!]
\begin{subequations} \label{eq:P2}
\begin{align} 
%&\hspace*{-3mm}\texttt{Stage-1 MPC Controller} & \notag\\
& \hspace*{-2.5mm} ~~\underset{\{\boldsymbol{u^1}, \boldsymbol{b^{GC}} \}}{\min} ~\mathcal{J}^{1} = w\mathcal{J}^{1}_\text{GC} +  \mathcal{J}^{1}_\text{CE} &  \hspace*{-5mm} \label{eq:P2_0} \\
&\hspace*{-3mm}\textbf{subject to: $\tau \in \{0,..,T^1-1\}$} ~  &\nonumber\\
&\hspace*{-3mm} \boldsymbol{x}^1_{t+\tau+1|t} = \Phi \boldsymbol{x}^1_{t+\tau|t} + \Gamma \boldsymbol{u}^1_{t+\tau|t}, & \hspace*{-5mm} \forall \tau \label{eq:P2_1}\\
&\hspace*{-3mm} \boldsymbol{x}^1_{t|t} = \boldsymbol{x}^1_{t|t-1},&\label{eq:P2_2}\\
&\hspace*{-3mm} b^{\text{G}}_{\kappa,t+\tau+1|t} = 1 \iff  \text{pos}(\boldsymbol{x}^1_{t+\tau+1|t}) \in  \bigtriangleup(S_\kappa), & \hspace*{-7mm} \forall \kappa, \tau \label{eq:P2_3}\\
&\hspace*{-3mm} \sum_\tau b^{\text{G}}_{\kappa,t+\tau+1|t} \leq 1 , & \hspace*{-7mm} \forall \kappa \label{eq:P2_3b}\\
&\hspace*{-3mm} \hat{b}^{\text{G}}_{\kappa,t+\tau+1|t} \leq  b^{\text{G}}_{\kappa,t+\tau+1|t} + V(\kappa), & \hspace*{-7mm} \forall \kappa, \tau \label{eq:P2_4}\\
&\hspace*{-3mm} C_m =  R_z(\phi^z)R_y(\phi^y)C_0,  & \hspace*{-15mm} \forall \{\phi^z,\phi^y\}\in \tilde{\mathcal{M}}\label{eq:P2_5}\\
&\hspace*{-3mm} \hat{C}_{m,t+\tau+1|t} = C_m+ \text{pos}(\boldsymbol{x}^1_{t+\tau+1|t}), & \hspace*{-5mm} \forall m, \tau \label{eq:P2_6}\\
&\hspace*{-3mm} b^{\text{FOV}}_{\kappa,m,t+\tau+1|t} = 1 \iff  \boldsymbol{c}_K \in  \bigtriangleup(\hat{C}_{m,t+\tau+1|t}), & \hspace*{-7mm} \forall \kappa, m, \tau \label{eq:P2_7}\\
&\hspace*{-3mm} \sum_\kappa \sum_m b^{\text{FOV}}_{\kappa,m,t+\tau+1|t} \leq 1, & \hspace*{-7mm} \forall \tau \label{eq:P2_8}\\
&\hspace*{-3mm} b^{GC}_{\kappa,m,t+\tau+1|t} = \hat{b}^{\text{G}}_{\kappa,t+\tau+1|t} \wedge b^{\text{FOV}}_{\kappa,m,t+\tau+1|t}, & \hspace*{-7mm} \forall \kappa, m, \tau \label{eq:P2_9}\\
&\hspace*{-3mm}  b^{GC}_{\kappa,m,t+\tau+1|t}, b^{\text{G}}_{\kappa,t+\tau+1|t}, \hat{b}^{\text{G}}_{\kappa,t+\tau+1|t} \in \{0,1\} & \hspace*{-7mm} \forall \kappa, \tau \\ 
&\hspace*{-3mm}  b^{\text{FOV}}_{\kappa,m,t+\tau+1|t}, V(\kappa) \in \{0,1\} & \hspace*{-7mm} \forall \kappa, \tau, m\\ 
&\hspace*{-3mm}  m \in \{1,..,|\tilde{\mathcal{M}|}\}, \kappa \in \{1,..,|\mathcal{\tilde{K}}_c|\} &\\
&\hspace*{-3mm} \boldsymbol{x}^1_{t|t}, \boldsymbol{x}^1_{t+\tau+1|t} \in \mathcal{X}^1,~ \boldsymbol{u}_{t+\tau|t}^1 \in \mathcal{U}^1 & \hspace*{-7mm} \forall \tau
\end{align}
\end{subequations}
\end{algorithm}


In \eqref{eq:P2}, we generate an ideal coverage reference plan based on simplified linear dynamics of the agent in a disturbance free setting, as shown in \eqref{eq:P2_1}, where the matrices $\Phi$ and $\Gamma$ are given by:
\begin{equation}
\Phi = 
\begin{bmatrix}
    \boldsymbol{1}_{3\times3} & \Delta_t^1\boldsymbol{1}_{3\times3}\\
    \boldsymbol{0}_{3\times3} &  \boldsymbol{1}_{3\times3}
   \end{bmatrix}, ~
\Gamma = 
\begin{bmatrix}
    \boldsymbol{0}_{3\times3} \\
    \boldsymbol{1}_{3\times3}
   \end{bmatrix}.
\end{equation}

\noindent The matrices  $\boldsymbol{1}_{3\times3}$ and $\boldsymbol{0}_{3\times3}$ denote the 3-by-3 identity and zero matrices respectively, and $\Delta_t^1$ denotes the sampling rate. The agent's state $\boldsymbol{x^1_{t}}$ is composed of position and velocity components in 3D Cartesian coordinates, and the control input vector $\boldsymbol{u^1_{t}}$ represents the velocity components in 3D coordinates. 
\subsubsection{Assumption 2:} For each point of interest $\boldsymbol{c}_K \in \tilde{\mathcal{K}}_c$, there is an associated region of interest $S_\kappa \subset \mathcal{A}$ (where $\kappa$ is the index used to identify $\boldsymbol{c}_K$). When the agent resides within this region (i.e., $\text{pos}(\boldsymbol{x}_{t}) \in S_\kappa$), there exist at least one configuration of the camera FOV $\hat{m} \in \{1,..,|\mathcal{M}|\}$ that can ensure the coverage of $\boldsymbol{c}_K$. $S_\kappa$ is identified as a sphere with radius $s_r$ centered at $\boldsymbol{\bar{s}}_\kappa = \ell\boldsymbol{a}^S_\kappa+\boldsymbol{c}_K$, where $\ell$ is a appropriately selected distance, and $\boldsymbol{a}^S_\kappa$ is the outward unit normal vector to the facet $K \in  \tilde{\mathcal{K}}$ which has as its centroid point, the point of interest $\boldsymbol{c}_K$. 

\textbf{UAV guidance through the regions of interest:} We utilize the binary variable $b^{\text{G}}_{\kappa,t+\tau+1|t}$ in \eqref{eq:P2_3} to identify whether the agent's position $\text{pos}(\boldsymbol{x}^1_{t+\tau+1|t})$ at the time-step $t+\tau+1|t$ inside the planning horizon (hereafter abbreviated as $\tau$) resides inside the convex-hull of the $\kappa_\text{th}$ sphere $S_\kappa$, associated with the point of interest $\boldsymbol{c}_K$. To implement this functionality with linear inequalities, we first convexify $S_\kappa$ by approximating it with the inscribed dodecahedron as in \cite{Papaioannou_jamming}. Subsequently, we can identify the presence of the agent inside the dodecahedron as shown below:
\begin{subequations}\label{eq:v0}
\begin{align} 
&  \text{dot}(\boldsymbol{a}_{i,\kappa},\text{pos}(\boldsymbol{x}^1_{\tau})) + \bar{b}^{\text{G}}_{i,\kappa,\tau}(M-\beta_{i,\kappa}) \le M, \label{eq:v1}\\
& 12 b^{\text{G}}_{\kappa,\tau} - \sum_{i=1}^{12}\bar{b}^{\text{G}}_{i,\kappa,\tau} \le 0 \label{eq:v2}
\end{align}
\end{subequations}
\noindent where $\text{dot}(\boldsymbol{a}_{i,\kappa},\boldsymbol{x})=\beta_{i,\kappa}$ describes the equation of the plane which contains the $i_\text{th}$ facet of the $\kappa_\text{th}$ dodecahedron associated with the point of interest $\boldsymbol{c}_K$, $\boldsymbol{x} \in \mathbb{R}^3$, $\text{dot}(a,b)$ is the dot product between the vectors $a$ and $b$, and $M$ is a sufficiently large positive constant that makes sure that \eqref{eq:v1} remains valid for any value of the binary decision variable $\bar{b}^{\text{G}}_{i,\kappa,\tau} \in \{0,1\}, \forall i \in \{1,..,12\}, \kappa, \tau$. Therefore, when the agent positional vector $\text{pos}(\boldsymbol{x^1_{\tau}})$ resides inside the convex-hull, of the $\kappa_\text{th}$ dodecahedron at time-step $\tau$ then the binary variable $\bar{b}^{\text{G}}_{i,\kappa,\tau}=1, \forall i$. Subsequently, the binary variable $b^{\text{G}}_{\kappa,\tau}$ can be utilized as shown in \eqref{eq:v2} to drive the agent inside the region of interest $S_\kappa$ at time-step $\tau$ (i.e., $b^{\text{G}}_{\kappa,\tau}=1$).
The constraint expressed in \eqref{eq:P2_3b} ensures that the agent generates plans that visit each region of interest exactly once within the planning horizon, and subsequently, the constraint in \eqref{eq:P2_4} makes sure that the agent avoids the duplication of work. If the agent has visited the region of interest $S_\kappa$ at some point in time, as indicated by $V(\kappa) \in \{0,1\}$ (i.e., a database that records the visited regions of interest), then according to \eqref{eq:P2_4}, there is no incentive to activate the variable $b^{\text{G}}_{\kappa,\tau}$ for the same region at a future time-step. Consequently, the agent generates coverage plans focusing on unvisited regions, thereby avoiding duplication of effort


\textbf{FOV control:} In this stage, to determine the camera rotations that allows the coverage of the points of interest $\boldsymbol{c}_\kappa, \forall \kappa  \in \{1,..,\tilde{\mathcal{K}}_c\}$, we plan hypothetical FOV configurations $m \in \{1,..,|\tilde{\mathcal{M}}|\}$ (i.e., assuming the camera gimbal can execute 1 out of $|\tilde{\mathcal{M}}|$ possible virtual rotations), without considering the orientation of the agent. Subsequently, we show in Sec. \ref{ssec:stage2}, how the stage-2 controller realizes the selected virtual FOV configurations by integrating the physical gimbal rotations $\mathcal{M}$ with robust control of the agent's orientation. 

The constraint in \eqref{eq:P2_5} pre-computes the camera FOV state $C_m$ for all possible virtual FOV configurations $m \in \{1,..,|\tilde{\mathcal{M}}|\}$, and subsequently \eqref{eq:P2_6} translates at time-step $\tau$ the camera FOV $\hat{C}_{m,t+\tau+1|t}$ in the predicted agent position i.e., $\text{pos}(\boldsymbol{x}^1_{t+\tau+1|t})$. Then, the binary variable $b^{\text{FOV}}_{\kappa,m,t+\tau+1|t}$ in \eqref{eq:P2_7} is activated when the point of interest $\boldsymbol{c}_K$ (indexed by $\kappa$) resides within the convex-hull of the $m_\text{th}$ virtual camera FOV at time-step $\tau$. This functionality is implemented similarly to \eqref{eq:v0} accounting for the 5 facets of the camera FOV. Constraint, \eqref{eq:P2_8} makes sure that only one FOV configuration is active at any point in time, and finally the logical conjunction in \eqref{eq:P2_9} integrates the guidance and coverage decision variables. In order, to generate the coverage plan over the rolling planning horizon we simultaneously optimize guidance and coverage as $\mathcal{J}^{1}_{GC} = - \sum_{\kappa=1}^{|\tilde{\mathcal{K}}_c|} \sum_{m=1}^{|\tilde{\mathcal{M}}|} \sum_{\tau=0}^{T^1-1} b^{GC}_{\kappa,m,t+\tau+1|t}$, as shown in \eqref{eq:P2_0}. The control effort denoted as $\mathcal{J}^{1}_{CE}$ has been defined in \eqref{eq:objective_P1}. A weighting scheme to balance the two sub-objectives can be adopted through the tuning parameter $w$.

In essence, the stage-1 controller generates the agent's trajectory $\{\boldsymbol{x}^1_{t+1|t},..,\boldsymbol{x}^1_{t+T^1|t}\}$, and a set of camera views $\{\hat{C}_{m_1,t+1|t},...,\hat{C}_{m_n,t+T^1|t}\}, m_i \in \{1,..,|\tilde{\mathcal{M}}|\}$ that maximize the coverage of the points of interest inside the planning horizon. We should note here that the agent's trajectory determines the order in which the various points of interest will be covered (i.e., a list which contains the sequence of coverage events obtained via $b^{GC}_{\kappa,t+\tau+1|t}$). The first element in this list (i.e., the point of interest which has been planned to be covered next), is passed as input to the stage-2 controller.


\subsection{Stage-2: Robust non-Gaussian Control} \label{ssec:stage2}

At each time-step, the stage-2 controller receives from stage-1 the region of interest $S_\kappa$ for some $\kappa \in \{1,..,|\tilde{\mathcal{K}}_c|\}$, which is planned to be visited next, and the selected virtual FOV associated to $S_\kappa$, which must be used to cover the corresponding point of interest. Subsequently, the objective of the stage-2 controller is to guide the agent robustly within $S_\kappa$ ensuring the correct agent orientation, i.e., an orientation that allows the on-board camera to match the virtual FOV configuration $m$, with $m \in \{1,..,|\tilde{\mathcal{M}}|\}$, selected in \eqref{eq:P2}. Such objective is attained by optimizing the agent's control inputs $\boldsymbol{u}_{t+\tau|t}$ according to \eqref{eq:nonlin_dynamics} over a suitably chosen planning horizon i.e., $\tau \in \{0,..,T-1\}$ of length $T$ time-steps. To achieve this goal, we employ exact uncertainty propagation techniques of mixed-trigonometric-polynomial functions, \cite{han2022non}, to effectively manage the external disturbances.


\subsubsection{Lemma 1:}
Consider a random variable $x$ with the characteristic function denoted by $\Phi_x(t)$. For a given triplet $(\alpha_1,\alpha_2,\alpha_3) \in \mathbb{N}^3$, where $\alpha = \sum_{i=1}^3 \alpha_i$, and a scaling factor $\delta$, the mixed-trigonometric-polynomial moment of order $\alpha$ of the form $\mu_{\delta,x^{\alpha_1} c^{\alpha_2}_x s^{\alpha_3}_x}$, is defined as $\mathbb{E}[(\delta x)^{\alpha_1} \cos^{\alpha_2}(\delta x) \sin^{\alpha_3}(\delta x)]$, and can be computed as:    
\begin{equation}\label{eq:lemma_1}
\begin{aligned}
\mu_{\delta,x^{\alpha_1} c^{\alpha_2}_x s^{\alpha_3}_x}= & \frac{1}{\iu^{(\alpha_1+\alpha_3)}2^{(\alpha_2+\alpha_3)}} \sum_{g=0}^{\alpha_2}\sum_{h=0}^{\alpha_3}\binom{\alpha_2}{g}\binom{\alpha_3}{h}\\
 & (-1)^{(\alpha_3-h)}\frac{\partial^{\alpha_1}}{\partial t^{\alpha_1}}\Phi_x(\delta\hspace{0.5mm}t)|_{t=2(g+h)-\alpha_2-\alpha_3}.
\end{aligned}
\end{equation}
\noindent The proof can be found in \cite{jasour2021moment}. We can now utilize this result in order to propagate the disturbance through the agent's nonlinear dynamics in \eqref{eq:nonlin_dynamics}, and compute the moments of the uncertain states. The agent's dynamics in \eqref{eq:nonlin_dynamics} can equivalently be written in the following form:
\begin{equation} \label{eq:aug_dynamics}
	\hat{\boldsymbol{x}}_t = A_{t-1} \hat{\boldsymbol{x}}_{t-1} + B_{t-1},
\end{equation}
\noindent where $\hat{\boldsymbol{x}}_t = [x_t,y_t,z_t,\cos(\psi_t),\sin(\psi_t)]^\top$, and using the fact that:
\begin{equation}
\begin{aligned}
    \cos(\psi_t) &=  \cos(\psi_{t-1})\cos(\Delta_t(u^\psi_{t-1}+\omega^\psi_{t-1}))\\
    &\quad -\sin\psi_{t-1}\sin(\Delta_t(u^\psi_{t-1}+\omega^\psi_{t-1})) \\
	\sin(\psi_t) &=  \sin(\psi_{t-1})\cos(\Delta_t(u^\psi_{t-1}+\omega^\psi_{t-1}))\\
	&\quad +\cos(\psi_{t-1})\sin(\Delta_t(u^\psi_{t-1}+\omega^\psi_{t-1})).
\end{aligned}
\end{equation}
$A_t$ and $B_t$ are given by:
\begin{equation}
A_t =
\begin{bmatrix}
  	1 & 0 & 0 & \Delta_t(u^\nu_y\mathord{+}\omega^\nu_t) & 0 \\
    0 & 1 & 0 & 0 & \Delta_t(u^\nu_t\mathord{+}\omega^\nu_t) \\
    0 & 0 & 1 & 0 & 0 \\
    0 & 0 & 0 & \cos(\Delta_t(u^\psi_t\mathord{+}\omega^\psi_t)) & -\sin(\Delta_t(u^\psi_t\mathord{+}\omega^\psi_t)) \\
    0 & 0 & 0 & \sin(\Delta_t(u^\psi_t\mathord{+}\omega^\psi_t)) & \cos(\Delta_t(u^\psi_t\mathord{+}\omega^\psi_t)) \\
\end{bmatrix},
\end{equation}
and $B_t = [0,0, \Delta_t(u^z_t+\omega^z_t),0,0]^\top$. With this transformation, \eqref{eq:lemma_1} can be directly applied to \eqref{eq:aug_dynamics}, to compute the first moment $\boldsymbol{\mu}^1_t$ of the uncertain state $\hat{\boldsymbol{x}}_t$ in a recursive fashion as a linear combination of mixed-trigonometric-polynomial functions of the disturbance term $\boldsymbol{\omega}_t = [\omega^\nu_t, \omega^z_t, \omega^\psi_t]$, and the control inputs $\boldsymbol{u}_t = [u^\nu_t, u^z_t, u^\psi_t]$. To see this observe that $\boldsymbol{\mu}^1_t = \mathbb{E}[\hat{\boldsymbol{x}}_t]$ and so
 $\boldsymbol{\mu}^1_t = [\mathbb{E}[x_t], \mathbb{E}[y_t],\mathbb{E}[z_t], \mathbb{E}[\cos(\psi_t)], \mathbb{E}[\sin(\psi_t)]]^\top$. Subsequently, applying the expectation operator to \eqref{eq:aug_dynamics} we obtain the moment-state dynamics as:
\begin{equation}\label{eq:first_moment}
\boldsymbol{\mu}^1_t = A^{mom_1}_{t-1} \boldsymbol{\mu}^1_{t-1} + B^{mom_1}_{t-1},
\end{equation}
where $A^{mom_1}_{t-1}$ and $B^{mom_1}_{t-1}$ are computed by the application of \eqref{eq:lemma_1} as:
\begin{equation}
A^{mom_1}_t =
\begin{bmatrix}
  	1 & 0 & 0 & \Delta_t u^\nu_t + \mu_{\Delta_t,\omega^\nu} & 0 \\
    0 & 1 & 0 & 0 & \Delta_t u^\nu_t + \mu_{\Delta_t,\omega^\nu} \\
    0 & 0 & 1 & 0 & 0 \\
    0 & 0 & 0 & \gamma_t & -\lambda_t \\
    0 & 0 & 0 & \lambda_t & \gamma_t \\
\end{bmatrix}
\end{equation}
where $\gamma_t = \cos(\Delta_t u^\psi_t)\mu_{\Delta_t,c_{\omega^\psi}}-\sin(\Delta_t u^\psi_t)\mu_{\Delta_t,s_{\omega^\psi}}$, $\lambda_t = \sin(\Delta_t u^\psi_t)\mu_{\Delta_t,c_{\omega^\psi}}+\cos(\Delta_t u^\psi_t)\mu_{\Delta_t,s_{\omega^\psi}}$, and finally $B^{mom_1}_t=[0,0,\Delta_t u^z_t + \mu_{\Delta_t,\omega^z},0,0]^\top$. The mixed moments of order  $\alpha$ i.e., $\boldsymbol{\mu}^\alpha_t = \mathbb{E}[(\hat{\boldsymbol{x}}_t)^\alpha] $ are obtained following the same procedure.
The procedure described above allows us to compute the moments of the uncertain states of the agent for any random disturbance term which exhibits finite moments, by propagating a finite sequence of moments from the initial probability distributions through the nonlinear stochastic dynamical system. This results in the acquisition of the moments of the system's state probability distributions over a planning horizon. 

Subsequently, we can apply known inequalities from probability theory that offer bounds on the likelihood of a random variable falling within a specified range. Based on these bounds, we can design controllers that ensure the process remains within desired limits, maintaining a predetermined level of confidence.

\begin{thm}  
Let $x$ be a real valued unimodal random variable with finite expectation $\mathbb{E}[x]$, variance $\mathbb{E}[(x-\mathbb{E}[x])^2]$, and $r \ge 0$, the one-sided Vysochanskij-Petunin inequality is given by:
\begin{equation}\label{eq:VP_inequality}
P(x-\mathbb{E}[x]\geq r)\leq \frac{4}{9}\frac{\mathbb{E}[(x-\mathbb{E}[x])^2]}{r^2+\mathbb{E}[(x-\mathbb{E}[x])^2]}.
\end{equation}
and holds when $r^2\geq\frac{5}{3}\mathbb{E}[(x-\mathbb{E}[x])^2]$. The proof can be found in \cite{VP}.
\end{thm}

First, we want to make sure that the agent reaches the region of interest $S_\kappa$, i.e., a sphere with center $\boldsymbol{\bar{s}}_\kappa = [s^\kappa_x, s^\kappa_y, s^\kappa_z]^\top$, and radius $s_r$, at the final state $\hat{\boldsymbol{x}}_{t+T|t}$ within a suitable selected planning horizon $T$. Let us denote the squared euclidean distance between the position of the UAV at the final state $\text{pos}(\hat{\boldsymbol{x}}_{t+T|t}) = [x_T,y_T,z_T]^\top$ of the horizon and the center of the region of interest $\boldsymbol{\bar{s}}_\kappa$ as $d^\kappa_T = ||\text{pos}(\hat{\boldsymbol{x}}_{t+T|t}) - \boldsymbol{\bar{s}}_\kappa||^2_2$. Because, the position of the UAV is uncertain, $d^\kappa_T$ becomes a random variable and therefore we are interested computing the UAV control inputs such that the probability $P(d^\kappa_T \geq s_r^2) \leq \epsilon$ (i.e., the UAV is outside the region of interest with probability at most $\epsilon$) %$P(d^\kappa_T \leq S_r^2)$ is satisfied with some predetermined level of confidence. 
is satisfied with some predetermined level of confidence. To do that, we define $f^\kappa_T = s_r^2 - d^\kappa_T$ and we compute an upper bound on the probability $P(f^\kappa_T \leq 0)$ utilizing the Vysochanskij-Petunin inequality as:
\begin{equation} \label{eq:VP2}
P(f^\kappa_T \leq 0)\leq \frac{4}{9} \frac{\mathbb{E}[(f^\kappa_T)^2]-\mathbb{E}[f^\kappa_T]^2}{\mathbb{E}[f^\kappa_T]^2},
\end{equation}
\noindent which is valid when $\mathbb{E}[f^\kappa_T]\geq 0$ and $\mathbb{E}[f^\kappa_T]^2 \geq \frac{5}{8}\mathbb{E}[(f^\kappa_T)^2]$. This result has been obtained by applying \eqref{eq:VP_inequality} to the unimodal random variable $x = -f^\kappa_T$, and setting $ r= \mathbb{E}[f^\kappa_T]$. The inequality in \eqref{eq:VP2} establishes the upper bound on $P(f^\kappa_T \leq 0)$, as a function of $\mathbb{E}[f^\kappa_T]$ and of $\mathbb{E}[(f^\kappa_T)^2]$. By expanding $f^\kappa_T$ and $(f^\kappa_T)^2$, and applying the expectation operator on the result, the upper bound can be expressed in terms of the first four moments of the system states. For instance, $\mathbb{E}[f^\kappa_T]$ is computed as $\mathbb{E}[ (x_T-s^\kappa_x)^2 + (y_T-s^\kappa_y)^2 + (z_T-s^\kappa_z)^2 - s_r^2]$ which is equal to:
\begin{align} \label{eq:avg}
&\mathbb{E}[(x_T)^2]-2\mathbb{E}[x_T]s^\kappa_x+(s^\kappa_x)^2+ \notag \\
&\mathbb{E}[(y_T)^2]-2\mathbb{E}[y_T]s^\kappa_y+(s^\kappa_y)^2+ \notag \\
&\mathbb{E}[(z_T)^2]-2\mathbb{E}[z_T]s^\kappa_z+(s^\kappa_z)^2-s_r^2.
\end{align}

\noindent where the first moments of the UAV state shown in the example above have been computed recursively through the moment-state dynamics as shown in \eqref{eq:first_moment}. Required higher order moments (in our case of order up to $\alpha=4$ which are required by $\mathbb{E}[(f^\kappa_T)^2]$) are computed in a similar fashion. The second objective is to adjust the orientation $\psi_{t+T|t}$ of the agent so that the camera can execute the virtual FOV configuration $m$, as selected in \eqref{eq:P2}. For the selected virtual FOV configuration $m$, characterized by rotation angles $\{\phi^z, \phi^y\} \in \tilde{\mathcal{M}}$, and for each real camera configuration $\hat{m} \in \{1,..,|\mathcal{M}|\}$  characterized by rotation angles $\{\hat{\phi}^z, \hat{\phi}^y\} \in \mathcal{M}$, where $\hat{\phi}^z = \phi^z$, there exists an orientation of the agent that ensures that the on-board camera can adhere to the virtual configuration, effectively covering the point of interest associated with $S_\kappa$. Such orientation of the agent, denoted as $\psi_{\hat{m}}$, is achieved by aligning the real the camera configurations expressed in the local reference system with the selected virtual FOV configuration. In other words:
\begin{equation} \label{eq:agent_orientation}
\phi^y = \psi_{\hat{m}} + \hat{\phi}^y.
\end{equation}
Note here that \eqref{eq:agent_orientation} must be mapped inside the range $[-\pi,\pi]$. The existence of at least one real camera configuration matching the selected virtual configuration is guaranteed by Assumption 2. However, in general, there might be multiple real FOV configurations that match the selected virtual FOV configuration. Consequently, a set of agent orientations could be employed to effectively cover the points of interest in $S_\kappa$. Without loss of generality, among the potential agent orientations derived in \eqref{eq:agent_orientation}, the stage-2 controller selects the agent orientation, denoted as $\psi_\kappa$ hereinafter, that aligns more closely with the tangent to the trajectory determined by the stage-1 controller when visiting $S_\kappa$ (example in Fig. \ref{fig:fig2}). This choice matches the stage-1 controller's objective of minimizing control effort.
To robustly control as desired the orientation $\psi_{t+T|t}$ of the agent at the end of the planning horizon $T$, the stage-2 controller leverages the observation that any orientation within the carefully chosen range $[\psi_\kappa-\Delta\psi, \psi_\kappa+\Delta\psi]$ ensures that the FOV configuration $\hat{m} \in \{1,..,|\mathcal{M}|\}$ combined with the orientation $\psi_\kappa$ covers the points of interest $\boldsymbol{c}_K$. Consequently, because the orientation of the agent is uncertain, the stage-2 controller aims at computing the agent's control inputs in a way that ensures, with a predefined level of confidence, the alignment of the agent's orientation within such valid range, i.e., $P(\psi_\kappa - \Delta\psi \leq \psi_{t+T|t} \leq \psi_\kappa + \Delta\psi) \geq 1-\epsilon$. To achieve this, considering that $\Delta\psi$ must be reasonably small for the selected camera configuration to cover the points of interest, the following is satisfied:
\begin{align} 
	&\psi_\kappa - \Delta\psi \leq \psi_{t+T|t} \leq \psi_\kappa + \Delta\psi \implies \notag \\
	&\sin(-\Delta\psi)\leq\sin(\psi_{t+T|t}-\psi_\kappa)\leq\sin(\Delta\psi) \label{eq:orientation_stage2a}
\end{align}

In line with the stage-1 objective of minimizing control effort, adhering to \eqref{eq:orientation_stage2a} ensures that the agent's orientation resides within the intended range rather than any other valid range, e.g., $\psi_\kappa - \Delta\psi \pm \pi \leq \psi_{t+T|t} \leq \psi_\kappa + \Delta\psi \pm \pi$. Thus, \eqref{eq:orientation_stage2a} can be expressed as:
\begin{equation} \label{eq:orientation_stage2b}
|\sin(\psi_{t+T|t})\cos(-\psi_\kappa)+\cos(\psi_{t+T|t})\sin(-\psi_\kappa)| \leq \sin(\Delta\psi),
\end{equation}

\noindent providing a condition on $\sin(\psi_{t+T|t})$ and $\cos(\psi_{t+T|t})$ that drives the orientation of the agent. Hence, to guarantee $P(\psi_\kappa \mathord{-} \Delta\psi \leq \psi_{t+T|t} \leq \psi_\kappa \mathord{+} \Delta\psi) \geq 1\mathord{-}\epsilon$, we define $\sigma^\kappa_T = \sin(\Delta\psi) - \sin(\psi_{t+T|t})\cos(-\psi_\kappa) - \cos(\psi_{t+T|t})\sin(-\psi_\kappa)$ and $\xi^\kappa_T = \sin(\Delta\psi) + \sin(\psi_{t+T|t})\cos(-\psi_\kappa) + \cos(\psi_{t+T|t})\sin(-\psi_\kappa)$ and, similarly to \eqref{eq:VP2}, we compute upper bounds on the probabilities $P(\sigma^\kappa_T \leq 0)$ and $P(\xi^\kappa_T \leq 0)$ using the Vysochanskij-Petunin inequality as follows:
\begin{align} 
P(\sigma^\kappa_T \leq 0)\leq \frac{4}{9} \frac{\mathbb{E}[(\sigma^\kappa_T)^2]-\mathbb{E}[\sigma^\kappa_T]^2}{\mathbb{E}[\sigma^\kappa_T]^2}\label{eq:VP3_a}\\
P(\xi^\kappa_T \leq 0)\leq \frac{4}{9} \frac{\mathbb{E}[(\xi^\kappa_T)^2]-\mathbb{E}[\xi^\kappa_T]^2}{\mathbb{E}[\xi^\kappa_T]^2}.\label{eq:VP3_b}
\end{align}

By applying the expectation operator to $\sigma^\kappa_T$, $\xi^\kappa_T$, and to the expanded version of $(\sigma^\kappa_T)^2$ and of $(\xi^\kappa_T)^2$, the upper bounds can be expressed in terms of the first two moments of the system states. Specifically, the upper bounds are computed as a function of $\mathbb{E}[\sin(\psi_{t+T|t})]$, $\mathbb{E}[\cos(\psi_{t+T|t})]$, $\mathbb{E}[(\sin(\psi_{t+T|t}))^2]$, $\mathbb{E}[(\cos(\psi_{t+T|t}))^2]$, and $\mathbb{E}[\sin(\psi_{t+T|t})\cos(\psi_{t+T|t})]$, which have been computed recursively through the moment-state dynamics as shown in \eqref{eq:first_moment}. Now, when the upper bounds are limited to $\epsilon/2$, $P(|\sin(\psi_{t+T|t})\cos(-\psi_\kappa)+\cos(\psi_{t+T|t})\sin(-\psi_\kappa)| \geq \sin(\Delta\psi))\leq \epsilon-\epsilon^2/4$, and the probability that the uncertain orientation $\psi_{t+T|t}$ is in the valid range $\psi_\kappa - \Delta\psi \leq \psi_{t+T|t} \leq \psi_\kappa + \Delta\psi$ is of at least $1-\epsilon$.

Finally, the stage-2 controller solves the optimization problem shown in \eqref{eq:P3} to robustly guide with the desired orientation the agent inside $S_\kappa$ with probability at least $1 - \epsilon$.
\vspace{-5mm}
\begin{algorithm}[h!]
\begin{subequations} \label{eq:P3}
\begin{align} 
%&\hspace*{-3mm}\texttt{Stage-1 MPC Controller} & \notag\\
& \hspace*{-2.5mm} ~~\underset{\{\boldsymbol{u} \in \mathcal{U}\}} {\min} ~\mathcal{J}^{0} = \sum_{t=1}^T ||\boldsymbol{u}_{t-1}||_2^2 &  \hspace*{-5mm} \label{eq:P3_0} \\
&\hspace*{-3mm}\textbf{subject to: $\tau \in \{0,..,T-1\}$} ~  &\nonumber\\
&\hspace*{-3mm} \boldsymbol{\mu}^n_{t+\tau+1|t} = A^{mom_n}_{t+\tau|t} \boldsymbol{\mu}^n_{t+\tau|t} + B^{mom_n}_{t+\tau|t}, & \hspace*{-5mm} \forall n, \tau \label{eq:P3_1}\\
&\hspace*{-3mm} \boldsymbol{\mu}^n_{t|t} = \boldsymbol{\mu}^n_{t-1|t}, & \hspace*{-5mm} \forall n, \tau \label{eq:P3_2}\\
&\hspace*{-3mm} \frac{4}{9} \frac{\mathbb{E}[(f^\kappa_{t+T|t})^2]-\mathbb{E}[f^\kappa_{t+T|t}]^2}{\mathbb{E}[f^\kappa_{t+T|t}]^2} \leq \epsilon, & \hspace*{-5mm}  \label{eq:P3_3}\\
&\hspace*{-3mm} \frac{4}{9} \frac{\mathbb{E}[(\sigma^\kappa_{t+T|t})^2]-\mathbb{E}[\sigma^\kappa_{t+T|t}]^2}{\mathbb{E}[\sigma^\kappa_{t+T|t}]^2} \leq \epsilon/2, & \hspace*{-5mm}  \label{eq:P3_4}\\
&\hspace*{-3mm} \frac{4}{9} \frac{\mathbb{E}[(\xi^\kappa_{t+T|t})^2]-\mathbb{E}[\xi^\kappa_{t+T|t}]^2}{\mathbb{E}[\xi^\kappa_{t+T|t}]^2} \leq \epsilon/2, & \hspace*{-5mm}  \label{eq:P3_5}\\
&\hspace*{-3mm} n = \{1,..,4\} & \hspace*{-7mm}
\end{align}
\end{subequations}
\end{algorithm}










